Flareon: Stealthy any2any Backdoor Injection via Poisoned Augmentation

Open software supply chain attacks, once successful, can exact heavy costs in mission-critical applications. As open-source ecosystems for deep learning flourish and become increasingly universal, they present attackers previously unexplored avenues to code-inject malicious backdoors in deep neural network models. This paper proposes Flareon, a small, stealthy, seemingly harmless code modification that specifically targets the data augmentation pipeline with motion-based triggers. Flareon neither alters ground-truth labels, nor modifies the training loss objective, nor does it assume prior knowledge of the victim model architecture, training data, and training hyperparameters. Yet, it has a surprisingly large ramification on training -- models trained under Flareon learn powerful target-conditional (or "any2any") backdoors. The resulting models can exhibit high attack success rates for any target choices and better clean accuracies than backdoor attacks that not only seize greater control, but also assume more restrictive attack capabilities. We also demonstrate the effectiveness of Flareon against recent defenses. Flareon is fully open-source and available online to the deep learning community: https://github.com/lafeat/flareon.

==> tables/method_compare.tex <==
\begin{table}[h!]
\footnotesize
\renewcommand{\arraystretch}{1.4}
\centering
\begin{tabular}{p{2.5cm}<{\centering}||p{1.5cm}<{\centering}p{1.5cm}<{\centering}p{1.5cm}<{\centering}p{1.5cm}<{\centering}p{1.5cm}<{\centering}}
Attack &WaNet &LC & FOA-O &FOA-A &NARCISSUS \\
\hline
No auxiliary model & \Checkmark & $\bigcirc$ &\Checkmark  &\Checkmark  &\XSolidBrush\\
Label poisoning  & \textbf{Dirty} & \textbf{Clean}  & \textbf{Clean} & \textbf{Clean} & \textbf{Clean}\\
Attack ratio  & 10$\%$  &2.5$\%$     &8$\%$ &40$\%$ &0.05$\%$\\
Black-box &\XSolidBrush   &\XSolidBrush    &\Checkmark  &\Checkmark &\Checkmark\\
Any-to-any &\XSolidBrush   &\XSolidBrush   &\XSolidBrush  &\Checkmark&\XSolidBrush\\
Augmentation & \XSolidBrush  &$\bigcirc$   &\Checkmark  &\Checkmark &$\bigcirc$\\
CA ($\%$)&92.88   &92.14  &96.09 &95.39 &95.14\\
ASR ($\%$)&99.34  &80.62 &95.90 &99.16 &97.92\\
\end{tabular}
\caption{Benchmark results on CIFAR-10 with ResNet-18 models and comparison of experimental setups.
``Attack ratio" indicates the ratio of attacked samples to all inputs.
``$\bigcirc$" denotes partial fulfillment of the requirement.
``Augmentation" indicates whether to consider the augmentation process.
``FOA-O" and ``FOA-A" represent any-to-one mode and any-to-any mode respectively.
}
\label{compare}
\end{table}

